Toward effective protection against diffusion based mimicry through score distillation

While generative diffusion models excel in producing high-quality images, they can also be misused to mimic authorized images, posing a significant threat to AI systems. Efforts have been made to add calibrated perturbations to protect images from diffusion-based mimicry pipelines. However, most of the existing methods are too ineffective and even impractical to be used by individual users due to their high computation and memory requirements. In this work, we present novel findings on attacking latent diffusion models (LDM) and propose new plug-and-play strategies for more effective protection. In particular, we explore the bottleneck in attacking an LDM, discovering that the encoder module rather than the denoiser module is the vulnerable point. Based on this insight, we present our strategy using Score Distillation Sampling (SDS) to double the speed of protection and reduce memory occupation by half without compromising its strength. Additionally, we provide a robust protection strategy by counterintuitively minimizing the semantic loss, which can assist in generating more natural perturbations. Finally, we conduct extensive experiments to substantiate our findings and comprehensively evaluate our newly proposed strategies. We hope our insights and protective measures can contribute to better defense against malicious diffusion-based mimicry, advancing the development of secure AI systems. The code is available in https://github.com/xavihart/Diff-Protect

==> text/others.tex <==

\begin{itemize}
    \item Current gradient-based protection methods are expensive to run
    \item Current gradient-based protection methods cause artifacts 
    \item Current gradient-based protection methods can be easily purified even by simple JPEG-compression~\citep{sandoval2023jpeg}.
\end{itemize}





\subsection{Diffusion-based Defense}

Diffusion model can be used to do black box task agnostic defense, just to name a few:


\begin{itemize}
    \item (Defense AdvPatch) DIFFender
    \item (Defense AdvAttack) Nie et al.
\end{itemize}




\subsection{Diffusion-based AdvAttack}

\begin{itemize}
    \item Diff-PGD~\citep{diff-pgd} [2023.5]
    \item Diff-attack~\citep{diff-attack} [2023.5]
    \item Concept-attack~\citep{chen2023content} [2023.5]
    \item Effective-Diff-Attack [anonymous, NeurIPS2023 submission]
    
\end{itemize}



\subsection{Diffusion-based Artist Protection}
\begin{itemize}
    \item MIST~\citep{liang2023adversarial} [2023.2]
    \item Glaze~\citep{shan2023glaze} [2023.2]
    \item Salman et al.~\citep{salman2023raising} [2023.2]
    \item JPEG-based~\citep{sandoval2023jpeg} [2023.4]
    \item DWT-style [anonymous, NeurIPS2023 submission]
    \item Simple-Pattern [twitter]: Some quite simple perturbation patterns (e.g. stripe, repeat) are proved to be effective to fool the imitator such.
\end{itemize}


\section{Our Solution}

\begin{itemize}
    \item Skip gradient can make the generation faster and cheaper
    \item In-domain attack can help generate more realistic adversarial samples
\end{itemize}

